Proving Termination Starting from the End

We present a novel technique for proving program termination which introduces a new dimension of modularity. Existing techniques use the program to incrementally construct a termination proof. While the proof keeps changing, the program remains the same. Our technique goes a step further. We show how to use the current partial proof to partition the transition relation into those behaviors known to be terminating from the current proof, and those whose status (terminating or not) is not known yet. This partition enables a new and unexplored dimension of incremental reasoning on the program side. In addition, we show that our approach naturally applies to conditional termination which searches for a precondition ensuring termination. We further report on a prototype implementation that advances the state-of-the-art on the grounds of termination and conditional termination.

==> summary.tex <==
% ;; -*- coding: iso-latin-1; TeX-PDF-mode: t; TeX-master: "main" -*-%

\section{ Brief summary of the 2nd phase}


\begin{theorem} Let $\psi$ be a set of states such it is not possible
  to start from a state in $\psi$, and after some time visit only
  states from $\varphi$. Then, $R$ terminates for any state in $\psi$.
  An alternative formulation is that any execution path that starts in
  a state from $\psi$, will have to periodically visit $\neg\varphi$.
\end{theorem}

\noindent
Let $\Phi=\mathit{gfp}\lambda Y. \varphi \cap \mathit{pre}[R](Y)$. The
set of states $\Phi$ is exactly the set of all states that if we start
from, then it is possible to always stay $\varphi$ (right from the
beginning). Our aim to avoid reaching such states.
%
Let $\Psi=\mathit{lfp}\lambda Z. \Phi \cup \mathit{pre}[R](Z)$. The set
of states $\Psi$ is the set of all states that can reach a state in
$\Phi$. 
%
This means that if we start from a state in $\psi=\neg\Psi$, then we
will not reach any state in $\Phi$, and thus we cannot stay in
$\varphi$, which means that $R$ terminates for $\psi$. Taking an
over-approximation of $\Phi$ and $\Psi$ is enough.

\bigskip
\noindent
How this is related to what Andrey does? 
%
\begin{enumerate}
\item As mentioned above, $\neg\varphi$ is what Andrey calls $s$;
%
\item Andrey simply approximates $\Phi$ using $\varphi$ ($\neg s$ in
  his notation), and then computes an over-approximation of $\Psi$
  using \texttt{interproc}.
\end{enumerate}
%
We already discussed the difference in Step~1, what we do has many
advatages over what Andery does. As regards Step~2, he does not
compute any iteration in the $\mathtt{gfp}$, he simply takes iteration
$0$ which is already over-approximation $\Phi$.


\bigskip
\noindent
Let us see an example. Let $R=\{x>0, x'=x+y, y'=-2y\}$ and $W=\{x>0,
x'<x\}$. Using these $R$ and $W$ we firt compute $\varphi\equiv
\{x>0,y\ge 0\}$ ($\neg s$ of Andrey).
%
Andrey uses this $\varphi$ as an over-approximation of $\Phi$, and
then computes, using \texttt{interproc}, and over-approximation of
$\mathit{lfp}\lambda Z. \varphi \cup \mathit{pre}(Z)$. He gets $\{x
\ge 1,x+y\ge 1\}$. Taking the negation gives $x \le 0 \vee x+y \le 0$
which is a trivial precondition for termination, that guarantees to
stop after $0$ or $1$ iteration.
%
Let us see what we get when computing a tighter over-approximation of
$\Phi$:
%
\[
\begin{array}{l}
  \Phi_0 =  \{x>0, y \ge 0\} \\
  \Phi_1 =  \Phi_0 \cap \mathit{pre}(\Phi_0) 
              =  \Phi_0 \cap \{x>0 , y \le 0\}
              =  \{x>0, y = 0\}\\
  \Phi_2 =  \Phi_0 \cap \mathit{pre}(\Phi_1) 
            =  \{x>0, y = 0\}\\
\end{array}
\]
%
so we reached the gfp in two iterations. Now we compute an
over-approximation of $\mathit{lfp}\lambda Z. \{x>0, y = 0\} \cup
\mathit{pre}(Z)$, using \texttt{interproc} for example, and we get
$\{y=0, x\ge 1\}$. Its negation is $y\ne 0\vee x<0$, which is the
optimal precondition for termination.
 

